Model-Agnostic Multi-Agent Perception Framework

Existing multi-agent perception systems assume that every agent utilizes the same model with identical parameters and architecture. The performance can be degraded with different perception models due to the mismatch in their confidence scores. In this work, we propose a model-agnostic multi-agent perception framework to reduce the negative effect caused by the model discrepancies without sharing the model information. Specifically, we propose a confidence calibrator that can eliminate the prediction confidence score bias. Each agent performs such calibration independently on a standard public database to protect intellectual property. We also propose a corresponding bounding box aggregation algorithm that considers the confidence scores and the spatial agreement of neighboring boxes. Our experiments shed light on the necessity of model calibration across different agents, and the results show that the proposed framework improves the baseline 3D object detection performance of heterogeneous agents.

==> archived/commented.tex <==


%   \subfloat[Pointpillar\label{fig:relia_pointpillar_uncali}]{%
%     \resizebox{0.5\linewidth}{!}{%
%       \begin{tikzpicture}%
%         \node(a){\includegraphics[width=0.5\linewidth,height=0.3\linewidth]{images/relia_pointpillar_train_uncali.pdf}};%
%       \end{tikzpicture}%
%     }%
%   }%
%   \subfloat[Pixor\label{fig:relia_pixor_uncali}]{%
%     \resizebox{0.5\linewidth}{!}{%
%       \begin{tikzpicture}%
%         \node(a){\includegraphics[width=0.5\linewidth,height=0.3\linewidth]{images/relia_pixor_train_uncali.pdf}};%
%       \end{tikzpicture}%
%     }%
%   }%







% \textbf{Expected Calibration Error (ECE)}. While reliability diagrams are useful visual tools, it is more convenient to have a scalar summary statistic of calibration. Since statistics comparing two distributions cannot be comprehensive, previous works have proposed variants, each with a unique emphasis. One notion of miscalibration is the difference in expectation between confidence and accuracy, i.e.
% \begin{equation}
%   \underset{\hat{P}}{\mathbb{E}}[|\mathbb{P}(\hat{Y}=Y \mid \hat{P}=p)-p|]
%   \label{eq:ece}
% \end{equation}
% Expected Calibration Error\todo[Refs]{Cite (Naeini et al., 2015)} -- or ECE -- approximates \cref{eq:ece} by partitioning predictions into $M$ equally-spaced bins (similar to the reliability diagrams) and taking a weighted average of the bins' accuracy/confidence difference. More precisely,
% \begin{equation}
%   \mathrm{ECE}=\sum_{m=1}^{M} \frac{\left|B_{m}\right|}{n}\left|\operatorname{acc}\left(B_{m}\right)-\operatorname{conf}\left(B_{m}\right)\right|
% \end{equation}
% where $n$ is the number of samples. The difference between acc and conf for a given bin represents the calibration $g a p$ (red bars in reliability diagrams -- e.g. \cref{fig:relia_uncali}). We use $\mathrm{ECE}$ as the primary empirical metric to measure calibration.


% Logistic calibration was proposed by  to reduce over-fitting by introducing a strong inductive bias which considers only calibration maps of the following form:


% Monotonicity is enforced assuming that higher model output scores suggest higher probability to be positive.
% For easier interpretability we introduce the parameter $m=-\nicefrac{\delta}{\gamma}$.
% This implies $\delta=-m\gamma$, yielding the following alternative parameterization:
% \begin{equation}
%   \mu_{\text {logistic }}(s ; \gamma,-m \gamma)=\frac{1}{1+1 / \exp (\gamma \cdot(s-m))}.
% \end{equation}
% The parameter $m$ determines the value of $s$ for which the calibrated score is $0.5$; the slope of the calibration map at $s=m$ is $\nicefrac{\gamma}{4}$.

% Formally, let the input $X\in\mathcal{X}$ and label $Y\in\mathcal{Y}=\{0,1\}$ be random variables that follow a ground-truth generative distribution $p(X,Y)=p(Y|X)p(X)$.
% We denote the classification output of an object detector to be $f(X)=(\hat{Y},\hat{S})$, where $\hat{Y}$ is a class prediction and $\hat{S}$ is the associated confidence score.

% s=\mathbb{P}_{p(X,Y)}\left(\hat{Y}=Y \mid \hat{S}=s\right),~\forall{s}\in[0,1].

% In practice, approximations are necessary when measuring how well a model is calibrated.

% Formally, a scoring classifier is perfectly calibrated on a dataset if for each of its output score $s$ the portion of positive samples with model output score $s$ is equal to $s$.
% Denoting the samples in the dataset by $\mathbf{x}_{1},\dots,\mathbf{x}_{n}$ and their binary labels by $y_{1},\dots,y_{n}$, a model $f$ is calibrated on this dataset if for each of its possible outputs $s_{i}=f(x_{i})$ the following holds:
% \begin{equation}
%   s_{i}=\mathbb{E}\left[Y \mid f(X)=s_{i}\right],
%   \label{eq:well_calibrated}
% \end{equation}
% where the random variables $X, Y$ denote the features and labels of uniformly randomly drawn samples from the dataset.
% Label $Y=1$ and $Y=0$ stand for a positive and negative, respectively.

% For any fixed model $f$ there exists a uniquely determined calibration map which produces perfectly calibrated probabilities on the given dataset.
% That calibration map can be defined as $\mu\left(s_{i}\right)=\mathbb{E}\left[Y \mid f(X)=s_{i}\right]$.
% However, 
% Usually we do not want to learn perfect calibration maps on the training data, because this would over-fit and would be far from being calibrated on the test data.
% For example, if the model $f$ outputs a different score on each training sample, the training-perfect calibration map would produce only the $0/1$-probabilities $\mu(s_{i})=y_{i}$, which in most cases would be overly confident.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Reliability Diagram
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \input{tex/fig_relia_uncali}
% \noindent\textbf{Reliability Diagrams}
% \cref{fig:relia_uncali} shows a visual representation of model calibration~\cite{degroot1983comparison,niculescu2005predicting}.\todo[Fontsize]{Fontsize is too small.}
% These diagrams plot empirical accuracy as a function of confidence scores.
% If the model is perfectly calibrated (i.e., \cref{eq:well_calibrated} holds) then the diagram should plot the identity function.
% Any deviation from the perfect reliability curve indicates \emph{miscalibration}.
% To compute the empirical accuracy to estimate the expected accuracy, we group the confidence scores into $M$ interval bins and calculate the accuracy of each bin.
% Let $I_{m}$ be the set of indices of samples whose confidence score falls into the interval $B_{m}=\left(\frac{m-1}{M}, \frac{m}{M}\right]$. The empirical accuracy of bin $B_{m}$ is
% \begin{equation*}
%   \operatorname{acc}\left(B_{m}\right)=\frac{1}{\left|I_{m}\right|} \sum_{i \in I_{m}} \operatorname{\delta}\left(\hat{y}_{i}=y_{i}\right),
% \end{equation*}
% where $\hat{y}_{i}$ and $y_{i}$ are the predicted and true class labels for sample $i$.
% The empirical accuracy $\operatorname{acc}\left(B_{m}\right)$ is an unbiased and consistent estimator of $\mathbb{P}\left(\hat{Y}=Y \mid \hat{S} \in B_{m}\right)$.
% We define the average confidence within bin $B_{m}$ as
% \begin{equation*}
%   \operatorname{conf}\left(B_{m}\right)=\frac{1}{\left|I_{m}\right|} \sum_{i \in I_{m}} \hat{s}_{i}
% \end{equation*}
% where $\hat{s}_{i}$ is the predictive confidence for the $i$-th sample.
% $\operatorname{conf}\left(B_{m}\right)$ and $\operatorname{acc}\left(B_{m}\right)$ approximate the left-hand and right-hand sides of \eqref{eq:well_calibrated} respectively for bin $B_{m}$
% Therefore, a perfectly calibrated model will have $\operatorname{acc}\left(B_{m}\right)=\operatorname{conf}\left(B_{m}\right)$ for all $m \in\{1, \ldots, M\}$.
% Note that reliability diagrams do not display the proportion of samples in a given bin, and thus cannot be used to estimate how many samples are calibrated.
% To address this, we further put the sample count histogram under the reliability diagram in \cref{fig:relia_uncali} and and use the opacity to depict the sample count weighted calibration gap.
% To summarize the reliability diagram into scalars, we also compute the sample count weighted confidence (dotted vertical line) and accuracy (solid vertical line).
% \cref{fig:relia_uncali} is the reliability diagrams of the Pointpillar and Second object detectors computed on a calibration dataset used in our experiment.
% We can see that, before calibration, both models have significant reliability gaps indicated by the red bars.
% Specifically, the Second detector tends to be more confident than the Pointpillar detector.
% This can be clearly seen from the gap between the average confidence (dotted line) and the average accuracy (solid line). Therefore, uncertainty calibration is necessary before fusing the predictions from heterogeneous agents.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.8\linewidth]{images/sigmoid_family.pdf}
%     \caption{Logistic calibration map family with various parameters.}%
%     \label{fig:logistic}
% \end{figure}

% This work follows the Beta calibration proposed by \citet{kull2017beta}, but replaces the Beta distribution with Kumaraswamy distribution, which has a differentiable and closed-form CDF


% {\algrenewcommand\textproc{}
%   \begin{algorithm}[thbp]\small
%     % \setstretch{1.3}
%     \caption{Promotion-Suppression Aggregation}\label{alg:aggregation}
%     \hspace*{\algorithmicindent} \textbf{Arguments}: A set of bounding boxes $\mathcal{B}=\{b_{1},\dots,b_{N}\}$\\
%     \hspace*{\algorithmicindent}\hspace{48pt} A confidence scores vector $\mathbf{c}=[c_{1},\dots,c_{N}]$
%     \begin{algorithmic}[1] 
%       \State compute IoU matrix $\mathbf{U}\in[0,1]^{N\times{N}}$
%       \State compute the old entropy $H^{0}=\mathtt{entropy}(\mathbf{c})$
%       \For {$t=1,\dots,t_{\text{max}}$}
%         \For {each vertex $v_{i}$}
%           \State promotion using \cref{eq:promotion}: $c_{i}=c_{i}+m_{i}^{+}$
%           \State suppression using \cref{eq:suppression}: $c_{i}=c_{i}-m_{i}^{-}$
%         \EndFor
%         \State compute the updated entropy $H_{t}=\mathtt{entropy}(\mathbf{c})$
%         \If {$H_{t-1}-H_{t}<\epsilon$}
%           break
%         \EndIf
%       \EndFor
%         \State \textbf{return} binary indexing vector $\mathbf{c}$
%       \end{algorithmic} 
%     \end{algorithm}


% Specifically, we create connections among bounding boxes according to their IoUs.
% Let $\mathcal{B}=\{b_{1},\dots,b_{N}\}$ be the raw bounding box set before post-processing and $\mathbf{c}=[c_{1},\dots,c_{N}]$ be the calibrated confidence score vector.
% Each vertex is associated with a bounding box $b_{i}$ and a calibrated confidence score $c_{i}$.
% We draw an undirected edge between two vertices if the IoU of their boxes is larger than a threshold.

% \noindent\textbf{Message Passing}.




% To gradually segregate the winning candidates and candidates to be removed, each box receives promotion message from its ``allies'' and suppression message from the dominating neighbor at the current iteration.
% We define the allies of candidate $i$ to be the set of neighboring boxes that have a relatively high IoUs with box $i$.
% Each candidate first updates its score using the received promotion message before applying the suppression message.
% The rationale behind this update order is that a candidate with slightly lower value, but many supporting allies, can be more valuable than the current best candidate.
% We should avoid suppressing the value of such candidates before aggregating the information from its allies.
% The suppression message portionally decrease the value of the suppressed candidate instead of completely purge the value, akin to soft-NMS~\citep{bodla2017soft}.
% Repeating the promotion and suppression step will drive the confidence vector to an extreme binary vector.
% We measure the entropy of the confidence vector $H^{t}=-\sum_{n=1}^{N}c_{i}\log(c_{i})$ and stop the iterative process when the entropy reduction is small enough $H^{t-1}-H^{t}<\epsilon$.
% Algorithm\,\ref{alg:aggregation} gives the overview of PSA, and we will explain the promotion messages and suppression messages in the following paragraphs.

% \textbf{Promotion Messages}. We design the promotion messages to meet the following desiderata.
% \begin{itemize}
%   \item The values of candidates with more allies should be increased more.
%   \item Having high-value allies brings a candidate more significant promotion.
%   \item Allies from the same party would like to promote their strongest candidate to compete with candidates from other parties within the neighborhood.
% \end{itemize}
% Formally, the promotion message is defined as
% \begin{equation}
%   m_{i}^{+}=(1-c_{i})\frac{N_{a}}{N_{a}+1}\max_{v_{j}\in\mathcal{A},c_{j}<c_{i}}c_{j},
%   \label{eq:promotion}
% \end{equation}
% where $\nicefrac{N_{a}}{(N_{a}+1)}$ indicates that the current candidate only gets half the value of its best ally when the number of allies $N_{a}$ is one and gets the full value when $N_{a}$ approaches infinity.
% Note that, to elect the strongest candidate in a party, we only allow the promotion message to flow from low-value candidates to high-value candidates.
% This is implied by the $c_{j}<c_{i}$ constraint.
% The received promotion message can at most increase the current value by $1-c_{i}$ to ensure that all the values are in the range $[0,1]$ and the value vector can eventually converge to a binary vector.

% \textbf{Suppression Messages}. After aggregating the promotion message from allies, candidates in the same neighborhood compete with each other.
% The winner will ``softly'' suppress the values of other candidates.
% This is implemented by passing the suppression message from the current best candidate to the others:
% \begin{equation}
%   m_{i}^{-}=c_{i}\mathtt{IoU}(b_{i},b_{i}^{\star,t}),
%   \label{eq:suppression}
% \end{equation}
% where $b_{i}$ is the bounding box of the current candidate and $b_{i}^{\star,t}$ is the bounding box of the best candidate at the $t$-th iteration within the regime of node $v_{i}$.
% Similar to the promotion message, the suppresion message can at most decrease the value that $v_{i}$ currently have to keep updated values in $[0,1]$.



% where $\mathtt{I}(\cdot)$ is the indicator function.

% A model is {well-calibrated} if the confidence score matches the expectation of correctly predicting the labels.
% 
% Note that $s'$ is continuous so we cannot compute the expectation in \cref{eq:well_calibrated} exactly using finite number of samples.
% In practice, $s'$ is discretized into several interval bins and we approximate \cref{eq:well_calibrated} using the empirical accuracy.

% \input{tex/fig_relia_uncali}
% \noindent\textbf{Uncertainty calibration evluation}.
% \cref{fig:relia_uncali} shows that reliability diagram of the Pointpillar object detector.
% In a reliability diagram, a perfectly calibrated model will produce a diagonal reliability curve where the empirical accuracy matches the predictive confidence score.
% If the reliability curve is under the diagonal line, the model is over-confident.
% Curves above the diagonal line indicates that the model under-estimates its accuracy.
% % Pointpillar object detector has significant reliability gaps before calibration.
% Pointpillar is too ``humble'' -- it can ahiceve higher accuracy than its prediction confidence score.
% This is a problem when combining the results of Pointpillar with another inaccurate detector that tends to give over-confident scores.
% Therefore, uncertainty calibration is necessary before fusing the results of different models.

% and the information hidden in the bounding box regression.
% Furthermore, we observe that the standard Non-Maximum Suppression algorithm for bounding box aggregation does not make full use of all the shared information from other agents.
 % in the framework, 
%Recent works have came up with a variety of multi-agent perception algorithms  and achieve high accuracy while maintaining low bandwidth requirements, Multi-agent system has demonstrated a great potential to significantly improve the perception performance. Existing 
% to mitigate the misalignment of confidence scores among different models, all models first calibrate the scores on the same calibration dataset independently before sharing the detection proposals. The aggregated proposals are then filtered by a novel fusion strategy that not only considers the confidence scores but also the bounding box consistency. 



% \todo[Weizhe\&Hao]{Please help finish the left paragraph, we want to describe briefly 1) the schema of the whole strategy to protect privacy 2) the calibrator to handle hetergeniety 3) a better clustering algorithm to further improve the results.}


% As long as different companies follows the same data sharing standards and protocols, all of the connected agents can communicate the model outputs with each other, leading to better privacy protection and confidentiality without revealing model architectures or weights. 

% However, it strictly requires the model consistency between agents to prevent large feature domain gap, which is non-trivial to satisfy in reality because of the confidentiality and privacy concerns. Late fusion, on the other hand, poses


%\subsection{3D LiDAR Detection}

% To measure how the uncertainty of a neural network is calibrated, \citet{murphy1977reliability} provides \textit{reliability diagrams} as an intuitive visual evaluation.
% Expected Calibration Error (ECE)~\citep{guo2017calibration} summarizes the mismatch between prediction confidence and empirical accuracy into a scalar.

% As \citet{guo2017calibration} discovers that scaling methods like Platt scaling~\citep{platt1999probabilistic} and Temperature scaling\citep{guo2017calibration} can calibrate neural networks effectively, our proposed method follows the same fashion. 
% We adopt the Cumulative Density Functions (CDFs) of the Kumaraswamy distribution~\cite{kumaraswamy1980generalized} as the calibration function family in our scaling method.
% Kumaraswamy distribution is differentiable and closely related to the Beta distribution~\citep{kull2017beta} but has simpler closed-form CDFs.
% To the best of our knowledge, this simple but flexible function has not been introduced in the uncertainty calibration literature.

% Since popularized by the pioneering work of \citet{guo2017calibration}, scaling methods, such as Platt scaling~\citep{platt1999probabilistic}, temperature scaling\citep{guo2017calibration}, isotonic regression~\citep{zadrozny2002transforming}, and Beta calibration~\citep{kull2017beta}, have been widely used in calibrating neural networks.

% All modern object detectors follow a three-step recipe: (1) proposing a search space of windows, (2) scoring/refining the window with a classifier/regressor, and (3) merging windows that might belong to the same object.
% This last stage is commonly referred to as “non-maximum suppression” (NMS)

% Notice that during offline stage, each agent can train their calibrator separately and during online stage, they only share the predicted bounding boxes and confidence scores while keeping the models' architectures and parameters secret, which makes the whole process confidential and preserves the privacy of each agent. The calibrator seems invisible to other agents and the shared message doesn't reveal underline perception models and data, leading to more secure and robust cooperative sharing mechanism. 

% Object detectors output bounding box predictions and the corresponding confidence scores.
% Intuitively, one would expect that these confidence scores imply the likelihood of correct prediction -- if we assign $80\%$ confidence to $100$ predictions,  we would expect that $80\%$ of these predictions are actually correct.
% Intuitively, one would expect that these confidence scores imply the likelihood of correct prediction -- if we assign $80\%$ confidence to $100$ predictions,  we would expect that $80\%$ of these predictions are actually correct.
% If this is the case, the classification model is said to be \emph{well-calibrated}.

    % \frac{\sum_{n=1}^{N}y_{n}\mathtt{I}(s=s')}{\sum_{n=1}^{N}\mathtt{I}(s=s')}=s',N\rightarrow\infty


% Since different models have distinct biases in confidence estimation, calibrators should be model-dependent.
% In our framework, all the agencies run their own object detectors on the same public object detection dataset to get a set of confidence scores and ground-truth labels.
% All the agencies build their calibration dataset from the same public object detection dataset.

% The scaling function $\mathtt{c}_{\bm{\theta}}(\tilde{s})$ cannot be an arbitrarily complex function, otherwise, the calibrator will overfit the calibration set which typically does not bring us better uncertainty calibration on the test set.
% We need to introduce some form of \emph{inductive bias} to regularize the learning.

% (with two ending bounds 0 and 1).
% First, a higher confidence score should indicate a higher expected accuracy. Thus we require the scaling function to be \textit{monotonically non-decreasing}.
% Second, we would like to learn a smooth scaling function instead of a wiggling one to avoid overfitting to the calibration set.
% Last but not least, the scaling function should be \textit{doubly bounded}, meaning that it maps a confidence interval $[0,1]$ to another valid confidence interval $[0,1]$.

% \input{tex/fig_spa.tex}
% In Non-Maximum Suppression (NMS), all candidate boxes are first sorted according to their confidence scores, and then the bounding box with the highest score in each cluster is selected as a representative.


% In this way, over-confident box proposals from neighboring vehicles can be filtered out based on its spatial agreement with proposals from connected agents. 


% PSA first constructs a graph based on the IoUs among candidates and their confidence scores.
% Then, all candidates with similar opinions (highly overlapped bounding boxes) propagate their values to each other as promotion messages.
% Finally, the most valuable candidate softly suppresses the values of other candidates to consolidate its dominance.
% The promotion and suppression steps are repeated until the entropy reduction of the value vector is small enough.
% The final value vector will be a binary vector that can be used to select the output bounding box.

% \noindent\textbf{Graph Building}.

% Moreover, to demonstrate the superiority of our proposed calibration method,
% we also evaluate other two other calibration approaches:  Platt Scaling~\cite{platt1999probabilistic}, and Temperature Scaling~\cite{guo2017calibration}. 


==> tex/fig_calibrators.tex <==
\begin{figure}[t]%
  \footnotesize
  \centering%
  \subfloat{%
    \resizebox{0.8\linewidth}{!}{
      \begin{tikzpicture}%
        \node at(0.0,0.0){\includegraphics[width=0.8\linewidth]{images/calibrator_benchmark.pdf}};%
        \node at (-1.8,-2.2) {TS};%
        \node at (0.3,-2.2) {PS};%
        \node at (2.3,-2.2) {DBS (Ours)};%
        \node[rotate=90] at (-3.5,0.0) {Average Precision ($\text{IoU}>0.7$)};%
      \end{tikzpicture}%
    }%
  }%
  \caption{\textbf{Comparison of different calibrators.}}%
  \label{fig:calibrators}
\end{figure}


==> tex/fig_kumaraswamy.tex <==
% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.8\linewidth]{images/kumaraswamy_family.pdf}
%     \caption{Kumaraswamy CDF calibration map family with various parameters}%
%     \label{fig:kumaraswamy}
% \end{figure}


==> tex/fig_relia_calied.tex <==
\begin{figure}[htbp]%
  \centering%
  \subfloat{%
    \resizebox{0.8\linewidth}{!}{
      \begin{tikzpicture}%
        \node at(0.0,0.0){\includegraphics[height=0.4\linewidth,width=\linewidth,trim={3 3 3 3},clip]{images/relia_pointpillar_train_kumaraswamy.pdf}};%
        \node at(0,-3){\includegraphics[height=0.2\linewidth,width=\linewidth,trim={3 3 3 3},clip]{images/confi_pointpillar_train_kumaraswamy.pdf}};%
        \node at(0.0,-4.2) {Confidence Scores};%
        \node at(-4.4,-1.6) {$0$};%
        \node at(-4.4,1.6) {$1$};%
        \node at(-4.4,-4.0) {$0$};%
        \node at(4.4,-4.0) {$1$};%
      \end{tikzpicture}%
    }%
  }%
  \caption{Reliability diagrams of Pointpillar after Kumaraswamy calibration.}\label{fig:relia_calied}%
%   \subfloat[Pixor]{%
%     \resizebox{0.5\linewidth}{!}{
%       \begin{tikzpicture}%
%         \node at(0.0, 0.0){\includegraphics[height=0.4\linewidth,width=\linewidth,trim={3 3 3 3},clip]{images/relia_pixor_train_kumaraswamy.pdf}};%
%         \node at(0, -3){\includegraphics[height=0.2\linewidth,width=\linewidth,trim={3 3 3 3},clip]{images/confi_pixor_train_kumaraswamy.pdf}};%
%         \node at(0.0,-4.2) {Confidence Scores};%
%         \node at(-4.4,-1.6) {$0$};%
%         \node at(-4.4,1.6) {$1$};%
%         \node at(-4.4,-4.0) {$0$};%
%         \node at(4.4,-4.0) {$1$};%
%       \end{tikzpicture}%
%     }%
%   }%
%   \caption{Reliability diagrams of the Pointpillar and Pixor object detection models after Kumaraswamy calibration.The legends are the same as in \cref{fig:relia_uncali}. Both models are \emph{well-calibrated} so the misalignment in the confidence scores are effectively eliminated. The average confidence (solid verticle line) can be used to filter out low-quality detection candidates after uncertainty calibration.}\label{fig:relia_calied}%
\end{figure}

% \begin{figure*}[t]%
%   \centering%
%   \subfloat[Pointpillar\label{fig:relia_pointpillar_kumaraswamy}]{%
%     \resizebox{0.5\linewidth}{!}{%
%       \begin{tikzpicture}%
%         \node(a){\includegraphics[width=0.5\linewidth,height=0.309\linewidth]{images/relia_pointpillar_train_kumaraswamy.pdf}};%
%       \end{tikzpicture}%
%     }%
%   }%
%   \subfloat[Ours on Pixor\label{fig:relia_pixor_kumaraswamy}]{%
%     \resizebox{0.5\linewidth}{!}{%
%       \begin{tikzpicture}%
%         \node(a){\includegraphics[width=0.5\linewidth,height=0.309\linewidth]{images/relia_pixor_train_kumaraswamy.pdf}};%
%       \end{tikzpicture}%
%     }%
%   }%
%   \caption{After Kumaraswamy calibration.}\label{fig:relia_calied}%
% \end{figure*}

  % \subfloat[Platt Scaling on Pointpillar\label{fig:relia_pointpillar_platt}]{%
  %   \resizebox{0.25\linewidth}{!}{%
  %     \begin{tikzpicture}%
  %       \node(a){\includegraphics[width=0.5\linewidth,height=0.309\linewidth]{images/relia_pointpillar_train_platt.pdf}};%
  %     \end{tikzpicture}%
  %   }%
  % }%

  % \subfloat[Platt Scaling on Pixor\label{fig:relia_pixor_platt}]{%
  %   \resizebox{0.25\linewidth}{!}{%
  %     \begin{tikzpicture}%
  %       \node(a){\includegraphics[width=0.5\linewidth,height=0.309\linewidth]{images/relia_pixor_train_platt.pdf}};%
  %     \end{tikzpicture}%
  %   }%
  % }%


==> tex/fig_spa.tex <==
\begin{figure*}[t]
  \centering
  \includegraphics[width=0.8\linewidth,height=0.3\linewidth]{example-image}
  \caption{Suppression-Promotion Aggregation.}%
  \label{fig:spa}
\end{figure*}


==> tex/tab_2.tex <==
% \begin{table}[htb]
%   \caption{Average precision at $0.5/0.7$ intersection over union of two different models.}\label{tab:diff_model}
%   \centering
%   \scriptsize
%   \begin{tabular}{
%       lll%
%     }
%     \toprule
%     Methods & {AP@IoU$>$0.5} & {AP@IoU$>$0.7}\\
%     % AP@IoU & 0.5\\
%     \midrule
%     None                                & 0.836 & 0.630\\
%     Platt Scaling                       & 0.852 & 0.715\\
%     Kumaraswamy Calibration             & 0.852 & 0.723\\
%     Intermediate fusion without calibration &0.716 &0.582\\
%     \bottomrule
%   \end{tabular}
% \end{table}

% \diagbox{Calibrator}{Aggregator}
% \multicolumn{2}{c}{NMS}
% & \multicolumn{2}{c}{IoU-NMS}
%  & 0.7 & 0.5 & 0.7
% \cmidrule(lr){2-3}\cmidrule(lr){4-5}
% & ? & ?
% & ? & ?
% & ? & ?
% &? &? 

% \begin{table}[htbp]
% \centering
% \caption{Ablation Study. Average Precision~(AP) at IoU=0.7 on \textit{Hetero1}.}
% \begin{tabular}{lll}
% \toprule
% \diagbox{Calibrators}{Aggregators} & NMS & PSA\\
% \midrule
% Temperature Scaling & 0.645 & 0.683\\
% Platt Scaling & 0.698 & 0.716\\
% Kumaraswamy Calibration & 0.713 & 0.720\\
% \bottomrule
% \end{tabular}
% \label{table:ablation}
% \end{table}

\begin{table}[htbp]
\centering
\caption{Calibrator performance. Expected Calibration Error (ECE) and Negative Log-Likelihood (NLL) of the calibrated Pixor detector evaluated on the calibration set and test set.}
\begin{tabular}{lllll}
\toprule
\diagbox{Calibrators}{Metrics} &
  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Calibration Set\\$\downarrow$ECE\hspace{10pt}$\downarrow$NLL\end{tabular}} &
  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Test Set\\$\downarrow$ECE\hspace{10pt}$\downarrow$NLL\end{tabular}}\\
\midrule
% Temperature Scaling     & 0.355 & 0.693 & 0.332 & 0.693\\
Platt Scaling           & 0.014 & 0.404 & 0.036 & 0.437\\
Kumaraswamy Scaling     & \textbf{0.004} & \textbf{0.403} & \textbf{0.028} & \textbf{0.434}\\
\bottomrule
\end{tabular}
\label{table:calibrator_comparison}
\end{table}


==> tex/tab_3.tex <==
\begin{table}[htbp]
  \centering
  \scriptsize
  \caption{Ablation study.}
  \begin{tabular}{llll}
    \toprule
    Calibrators & Aggregators &
    \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Hetero1\\ $\uparrow$AP@0.7\end{tabular}} &
    \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Hetero2\\ $\uparrow$AP@0.7\end{tabular}} \\
    \midrule
    N/A & NMS & 0.691 & 0.723\\
    Temperature & NMS & 0.423 & 0.480\\
    Platt Scaling & NMS & 0.724 & 0.766\\
    Ours & NMS & \textbf{0.734} & \textbf{0.776}\\
    \midrule
    N/A & PSA & 0.736 & 0.763\\
    Temperature & PSA & 0.691 & 0.522\\
    Platt Scaling & PSA & 0.749 & 0.771\\
    Ours & PSA & \textbf{0.750} & \textbf{0.784}\\
    \bottomrule
  \end{tabular}
  \label{table:calibrator_benchmark}
\end{table}

